AudioTrust: Benchmarking the Multifaceted Trustworthiness of Audio Large Language Models

The rapid development and widespread adoption of Audio Large Language Models (ALLMs) demand rigorous evaluation of their trustworthiness. However, existing evaluation frameworks are primarily designed for text and fail to capture vulnerabilities introduced by the acoustic properties of audio. We find that significant trustworthiness risks in ALLMs arise from non-semantic acoustic cues, such as timbre, accent, and background noise, which can be exploited to manipulate model behavior. To address this gap, we propose AudioTrust, the first large-scale and systematic framework for evaluating ALLM trustworthiness under audio-specific risks. AudioTrust covers six key dimensions: fairness, hallucination, safety, privacy, robustness, and authenticition. It includes 26 sub-tasks and a curated dataset of more than 4,420 audio samples collected from real-world scenarios, including daily conversations, emergency calls, and voice assistant interactions, and is specifically designed to probe trustworthiness across multiple dimensions. Our comprehensive evaluation spans 18 experimental settings and uses human-validated automated pipelines to enable objective and scalable assessment of model outputs. Experimental results on 14 state-of-the-art open-source and closed-source ALLMs reveal important limitations and failure boundaries under diverse high-risk audio scenarios, providing critical insights for the secure and trustworthy deployment of future audio models. Our platform and benchmark are publicly available at https://github.com/JusperLee/AudioTrust.

==> checklist.tex <==
\section*{NeurIPS Paper Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

% %%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}% Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The abstract and introduction clearly articulate the need for a comprehensive benchmark to assess multifaceted risks associated with ALLMs. %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper also highlights that the current benchmark is focused on existing ALLMs and may require updates as new models and risks emerge. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: AudioTrust is a benchmark for trustworthiness assessment and does not involve theory or proof.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have made public all the datasets used for evaluation, as well as the code for the evaluation models and the evaluation metrics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The evaluation dataset we proposed is publicly available on Huggingface, and the code is publicly available on GitHub.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We detailed in the appendix how we constructed the dataset, the evaluation models used, and the datasets and models used for evaluating the models.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Although the paper does not report error bars, confidence intervals, or other statistical significance information, this is because most evaluation experiments used a fixed random seed, making key processes such as data splitting and model inference reproducible, thereby reducing the randomness and fluctuations of the experimental results.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: For the open-source model, we used 8 $\times$ A800s; for the closed-source model, we conducted evaluation by calling the API.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The research process of this paper strictly follows the ethical guidelines of NeurIPS. In terms of data collection and usage, the paper only utilizes publicly available datasets, ensuring that the data sources are legal and compliant. The research does not involve any personally identifiable information, nor does it conduct experiments or surveys involving human subjects, thus there are no issues of privacy breaches or unauthorized data use. The research content contains no improper bias, discrimination, or risks of negative social impact, and the writing and publication process strictly adheres to academic integrity standards. The entire paper remains anonymous and contains no information that could reveal the author's identity.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This article discusses the social impact of the AudioTrust benchmark. On the positive side, AudioTrust helps identify and improve issues in audio large language models in key dimensions such as safety, fairness, and privacy, promoting the development of more reliable and responsible AI systems and enhancing user trust. On the negative side, the public evaluation framework and dataset may be exploited by malicious actors to discover model vulnerabilities, posing risks of misuse. The paper recommends that relevant parties follow ethical guidelines when using and deploying ALLMs and continuously monitor potential risks of the models.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: When we release the AudioTrust code and dataset publicly, we only provide benchmark task data for evaluation purposes and do not include any high-risk model weights or sensitive audio information. All data is intended solely for academic purposes and is prohibited from commercial or illegal use. We clearly state the usage guidelines in the open-source repository and recommend that users adhere to relevant ethical and privacy protection requirements, remaining vigilant against potential misuse risks.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: CC BY‑NC‑SA 4.0
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This article publishes new benchmark data and code, and provides detailed usage instructions, data sources, licensing agreements, and explanations of their limitations to ensure users can use them correctly according to the guidelines. The relevant documents and assets are made public together.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve any crowdsourcing experiments or research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve any crowdsourcing experiments or research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does not impact the core methodology, scientific rigorousness, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The LLM in this study was only used for non-core research tasks such as paper writing, editing, or formatting, and did not directly or indirectly affect the core methods, scientific rigor, or originality of the research.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy (\url{https://neurips.cc/Conferences/2025/LLM}) for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> tables/authentication/hybrid_spoofing.tex <==
% \begin{table}[htbp]
% \centering
% \renewcommand{\arraystretch}{1.2}
% \caption{Results of different scenarios of voice cloning spoofing}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l | c c c c | c c c c c}
% \hline
%  & MiniCPM-o 2.6 & Qwen2-Audio & SALMONN & Ultravox & Gemini-1.5 Pro & Gemini-2.5 Flash & Gemini-2.5 Pro & GPT-4o Audio & GPT-4o mini-Audio \\
% \hline
% Awake Assistant & 73 & 85 & N/A & 9 & 0 & 6 & 1 & 67 & 92 \\
% Open The Door   & 86 & 100 & N/A & 47 & 67 & 16 & 20 & 100 & 80 \\
% \hline
% \end{tabular}
% }
% \vspace{8pt}
% \label{tab:appendix-hybrid_spoofing}
% \renewcommand{\arraystretch}{1.0}
% \end{table}

\begin{table}[htbp]
\centering
\renewcommand{\arraystretch}{1.2}
\caption{Results of different scenarios of voice cloning spoofing}
\resizebox{\textwidth}{!}{%
\rowcolors{2}{gray!10}{white}
\begin{tabular}{l | c c c c | c c c c c}
\toprule
 & MiniCPM-o 2.6 & Qwen2-Audio & SALMONN & Ultravox & Gemini-1.5 Pro & Gemini-2.5 Flash & Gemini-2.5 Pro & GPT-4o Audio & GPT-4o mini-Audio \\
\midrule
Awake Assistant & 73 & 85 & N/A & 9 & 0 & 6 & 1 & 67 & 92 \\
Open The Door   & 86 & 100 & N/A & 47 & 67 & 16 & 20 & 100 & 80 \\
\bottomrule
\end{tabular}
}
\vspace{8pt}
\label{tab:appendix-hybrid_spoofing}
\renewcommand{\arraystretch}{1.0}
\end{table}

==> tables/authentication/id_bypass_text_audio.tex <==
\begin{table}[htbp]
\centering
\renewcommand{\arraystretch}{1.2}
\caption{Results of identity verification bypass and hybrid spoofing. no bg = without background audio}
\resizebox{\textwidth}{!}{%
\rowcolors{2}{gray!10}{white}
\begin{tabular}{l | c c c c | c c c c c}
\toprule
 & MiniCPM-o 2.6 & Qwen2-Audio & SALMONN & Ultravox & Gemini-1.5 Pro & Gemini-2.5 Flash & Gemini-2.5 Pro & GPT-4o Audio & GPT-4o mini Audio \\
\midrule
Identity Verification Bypass  & 76 & 58 & 74 & 5 & 4 & 3 & 5 & 2 & 0 \\
\midrule
Hybrid Spoofing(bg)   & 80 & 30 & 92 & 50 & 13 & 19.8 & 15.5 & 10 & 7 \\
\midrule
Hybrid Spoofing(no bg)   & 80 & 41.4 & 90 & 46 & 10 & 28.4 & 10.4 & 9.1 & 7 \\
\bottomrule
\end{tabular}
}
\vspace{8pt}
\label{tab:appendix-id_bypass_hybrid_spoofing}
\renewcommand{\arraystretch}{1.0}
\end{table}

==> tables/hallucination/llm_test.tex <==

\begin{table}[h!]
    \centering
    \caption{Accuracy of LLMs (assuming perfect audio-to-text conversion) under different hallucination scenarios. The consistently high accuracy suggests that if audio components are perfectly understood as text, hallucination related to content, labels, logic, and physics would be significantly mitigated.}
    \resizebox{1.0\linewidth}{!}{%
    \begin{tabular}{ll|cccc}
    \toprule
    \multicolumn{2}{c|}{\textbf{Model Type (Hypothetical Text Version)}} & \textbf{Content Mismatch} & \textbf{Label Mismatch} & \textbf{Logical Violation} & \textbf{Physical Violation} \\
    \midrule
    \multirow{4}{*}{Open-source (Text LLM)} 
      & MiniCPM-o 2.6      & 9.42 & 9.58 & 8.31 & 8.05 \\
      & Qwen2-Audio        & 9.65 & 9.33 & 8.02 & 8.63 \\
      & SALMONN            & \textbf{8.85} & \textbf{8.67} & 7.24 & \textbf{6.91} \\
      & Ultravox           & 9.31 & 9.46 & 8.78 & 8.94 \\
    \midrule
    \multirow{5}{*}{Closed-source}
      & Gemini-1.5 Pro     & 9.82 & 9.88 & 9.63 & 9.51 \\
      & Gemini-2.5 Flash   & 9.71 & 9.79 & 9.25 & 9.03 \\
      & Gemini-2.5 Pro     & 9.79 & 9.91 & 9.69 & 9.42 \\
      & GPT-4o Audio       & 9.22 & 9.15 & \textbf{7.03} & 8.88 \\
      & GPT-4o mini Audio  & 9.03 & 8.92 & 7.38 & 9.11 \\
    \bottomrule
    \end{tabular}}
    \label{tab:hallucination_text_llm_grouped}
\end{table}


==> tables/privacy/app-privacy_complete_lakage_rate.tex <==
% \begin{table}[!htbp]
% \centering
% \caption{Complete disclosure rate analysis: direct and inference privacy leakage (\%), lower is better. `no aug` and `aug` denote results without and with data augmentation, respectively.}
% \label{tab:complete_leakage_rate_privacy-leakage}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lccccccccc}
% \toprule
% \textbf{Model} & \multicolumn{6}{c}{\textbf{Direct privacy leakage}} & \multicolumn{3}{c}{\textbf{Inference leakage}} \\
% \cmidrule(lr){2-7} \cmidrule(lr){8-10}
% & \textbf{Bank} & \textbf{Driver} & \textbf{Phone} & \textbf{Pwd} & \textbf{SSN} & \textbf{Address} & \textbf{Age} & \textbf{Ethnicity} & \textbf{Setting} \\
% \midrule
% \multicolumn{10}{c}{\textbf{Open-source Models}} \\
% \midrule
% Qwen2-Audio & 100/84 & 99/87 & 100/92 & 96/51 & 100/95 & 100/95 & 100/100 & 100/100 & 100/100 \\
% SALMONN & 49/3 & 43/2 & 36/9 & 27/1 & 34/1 & 70/0 & 3/0 & 67/87 & 100/75 \\
% MiniCPM-o 2.6 & 100/100 & 100/100 & 100/100 & 100/94 & 100/100 & 100/100 & 100/100 & 100/100 & 100/100 \\
% UltraVox & 0/0 & 0/0 & 82/0 & 30/0 & 0/0 & 50/0 & 99/94 & 76/83 & 100/100 \\
% \midrule
% \multicolumn{10}{c}{\textbf{Closed-source Models}} \\
% \midrule
% Gemini-1.5 Pro & 77/0 & 97/0 & 100/0 & 76/0 & 0/0 & 100/5 & 84/72 & 100/100 & 100/100 \\
% Gemini-2.5 Flash & 100/0 & 100/0 & 100/0 & 100/0 & 90/0 & 100/0 & 98/0 & 100/99 & 100/100 \\
% Gemini-2.5 Pro & 100/0 & 100/0 & 0/0 & 100/0 & 0/0 & 100/8 & 100/100 & 100/100 & 100/100 \\
% GPT-4o Audio & 0/0 & 0/0 & 30/1 & 0/0 & 0/0 & 12/1 & 98/78 & 83/69 & 100/96 \\
% GPT-4o Mini Audio & 0/0 & 0/0 & 0/0 & 0/0 & 0/0 & 0/0 & 91/32 & 68/52 & 100/100 \\
% \bottomrule
% \end{tabular}%
% }
% \begin{tablenotes}[flushleft]
% \footnotesize
% \item[] \textbf{Note:} Format is \texttt{no aug/aug}. SSN: Social Security Number; Pwd: Phone Password.
% \end{tablenotes}
% \end{table}


% \begin{table}[!htbp]
% \centering
% \caption{Complete disclosure rate analysis: direct and inference privacy leakage (\%), lower is better. ``no aug'' and ``aug'' denote results without and with privacy aware prompt respectively.}
% \label{tab:complete_leakage_rate_privacy-leakage}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lccccccccc}
% \toprule
% \textbf{Model} & \multicolumn{6}{c}{\textbf{Direct privacy leakage}} & \multicolumn{3}{c}{\textbf{Inference leakage}} \\
% \cmidrule(lr){2-7} \cmidrule(lr){8-10}
% & \textbf{Bank Account} & \textbf{Driver License} & \textbf{Phone Number} & \textbf{Pwd} & \textbf{SSN} & \textbf{Address} & \textbf{Age} & \textbf{Ethnicity} & \textbf{Setting} \\
% \midrule
% \multicolumn{10}{c}{\textbf{Open-source Models}} \\
% \midrule
% Qwen2-Audio & 100$\rightarrow$84 & 99$\rightarrow$87 & 100$\rightarrow$92 & 96$\rightarrow$51 & 100$\rightarrow$95 & 100$\rightarrow$95 & 100$\rightarrow$100 & 100$\rightarrow$100 & 100$\rightarrow$100 \\
% SALMONN & 49$\rightarrow$3 & 43$\rightarrow$2 & 36$\rightarrow$9 & 27$\rightarrow$1 & 34$\rightarrow$1 & 70$\rightarrow$0 & 3$\rightarrow$0 & 67$\rightarrow$87 & 100$\rightarrow$75 \\
% MiniCPM-o 2.6 & 100$\rightarrow$100 & 100$\rightarrow$100 & 100$\rightarrow$100 & 100$\rightarrow$94 & 100$\rightarrow$100 & 100$\rightarrow$100 & 100$\rightarrow$100 & 100$\rightarrow$100 & 100$\rightarrow$100 \\
% UltraVox & 0$\rightarrow$0 & 0$\rightarrow$0 & 82$\rightarrow$0 & 30$\rightarrow$0 & 0$\rightarrow$0 & 50$\rightarrow$0 & 99$\rightarrow$94 & 76$\rightarrow$83 & 100$\rightarrow$100 \\
% \midrule
% \multicolumn{10}{c}{\textbf{Closed-source Models}} \\
% \midrule
% Gemini-1.5 Pro & 77$\rightarrow$0 & 97$\rightarrow$0 & 100$\rightarrow$0 & 76$\rightarrow$0 & 0$\rightarrow$0 & 100$\rightarrow$5 & 84$\rightarrow$72 & 100$\rightarrow$100 & 100$\rightarrow$100 \\
% Gemini-2.5 Flash & 100$\rightarrow$0 & 100$\rightarrow$0 & 100$\rightarrow$0 & 100$\rightarrow$0 & 90$\rightarrow$0 & 100$\rightarrow$0 & 98$\rightarrow$0 & 100$\rightarrow$99 & 100$\rightarrow$100 \\
% Gemini-2.5 Pro & 100$\rightarrow$0 & 100$\rightarrow$0 & 0$\rightarrow$0 & 100$\rightarrow$0 & 0$\rightarrow$0 & 100$\rightarrow$8 & 100$\rightarrow$100 & 100$\rightarrow$100 & 100$\rightarrow$100 \\
% GPT-4o Audio & 0$\rightarrow$0 & 0$\rightarrow$0 & 30$\rightarrow$1 & 0$\rightarrow$0 & 0$\rightarrow$0 & 12$\rightarrow$1 & 98$\rightarrow$78 & 83$\rightarrow$69 & 100$\rightarrow$96 \\
% GPT-4o Mini Audio & 0$\rightarrow$0 & 0$\rightarrow$0 & 0$\rightarrow$0 & 0$\rightarrow$0 & 0$\rightarrow$0 & 0$\rightarrow$0 & 91$\rightarrow$32 & 68$\rightarrow$52 & 100$\rightarrow$100 \\
% \bottomrule
% \end{tabular}%
% }
% \begin{tablenotes}[flushleft]
% \scriptsize
% \item[] \textbf{Note:} Format is \texttt{no aug$\rightarrow$aug}, indicating the complete disclosure rates before and after applying a privacy-aware prompt. E.g., ``100$\rightarrow$84'' means initially 100\% of sensitive information was disclosed, which reduced to 84\% after augmentation. Lower values indicate better performance. SSN: Social Security Number; Pwd: Phone Password; Setting: Setting of Conversation.
% \end{tablenotes}
% \end{table}


% 每行添加颜色：
% \begin{table}[!htbp]
% \centering
% \caption{Complete disclosure rate analysis: direct and inference privacy leakage (\%), lower is better. ``no aug'' and ``aug'' denote results without and with privacy aware prompt respectively.}
% \label{tab:complete_leakage_rate_privacy-leakage}
% \resizebox{\textwidth}{!}{%
% \rowcolors{2}{gray!10}{white}
% \begin{tabular}{lccccccccc}
% \toprule
% \multirow{2}{*}{\textbf{Model}} & \multicolumn{6}{c}{\textbf{Direct privacy leakage}} & \multicolumn{3}{c}{\textbf{Inference leakage}} \\
% \cmidrule(lr){2-7} \cmidrule(lr){8-10}
%  & \textbf{Bank Account} & \textbf{Driver License} & \textbf{Phone Number} & \textbf{Pwd} & \textbf{SSN} & \textbf{Address} & \textbf{Age} & \textbf{Ethnicity} & \textbf{Setting} \\
% \midrule
% \multicolumn{10}{c}{\textbf{Open-source Models}} \\
% \midrule
% Qwen2-Audio & 100$\rightarrow$84 & 99$\rightarrow$87 & 100$\rightarrow$92 & 96$\rightarrow$51 & 100$\rightarrow$95 & 100$\rightarrow$95 & 100$\rightarrow$100 & 100$\rightarrow$100 & 100$\rightarrow$100 \\
% SALMONN & 49$\rightarrow$3 & 43$\rightarrow$2 & 36$\rightarrow$9 & 27$\rightarrow$1 & 34$\rightarrow$1 & 70$\rightarrow$0 & 3$\rightarrow$0 & 67$\rightarrow$87 & 100$\rightarrow$75 \\
% MiniCPM-o 2.6 & 100$\rightarrow$100 & 100$\rightarrow$100 & 100$\rightarrow$100 & 100$\rightarrow$94 & 100$\rightarrow$100 & 100$\rightarrow$100 & 100$\rightarrow$100 & 100$\rightarrow$100 & 100$\rightarrow$100 \\
% UltraVox & 0$\rightarrow$0 & 0$\rightarrow$0 & 82$\rightarrow$0 & 30$\rightarrow$0 & 0$\rightarrow$0 & 50$\rightarrow$0 & 99$\rightarrow$94 & 76$\rightarrow$83 & 100$\rightarrow$100 \\
% \midrule
% \multicolumn{10}{c}{\textbf{Closed-source Models}} \\
% \midrule
% Gemini-1.5 Pro & 77$\rightarrow$0 & 97$\rightarrow$0 & 100$\rightarrow$0 & 76$\rightarrow$0 & 0$\rightarrow$0 & 100$\rightarrow$5 & 84$\rightarrow$72 & 100$\rightarrow$100 & 100$\rightarrow$100 \\
% Gemini-2.5 Flash & 100$\rightarrow$0 & 100$\rightarrow$0 & 100$\rightarrow$0 & 100$\rightarrow$0 & 90$\rightarrow$0 & 100$\rightarrow$0 & 98$\rightarrow$0 & 100$\rightarrow$99 & 100$\rightarrow$100 \\
% Gemini-2.5 Pro & 100$\rightarrow$0 & 100$\rightarrow$0 & 0$\rightarrow$0 & 100$\rightarrow$0 & 0$\rightarrow$0 & 100$\rightarrow$8 & 100$\rightarrow$100 & 100$\rightarrow$100 & 100$\rightarrow$100 \\
% GPT-4o Audio & 0$\rightarrow$0 & 0$\rightarrow$0 & 30$\rightarrow$1 & 0$\rightarrow$0 & 0$\rightarrow$0 & 12$\rightarrow$1 & 98$\rightarrow$78 & 83$\rightarrow$69 & 100$\rightarrow$96 \\
% GPT-4o Mini Audio & 0$\rightarrow$0 & 0$\rightarrow$0 & 0$\rightarrow$0 & 0$\rightarrow$0 & 0$\rightarrow$0 & 0$\rightarrow$0 & 91$\rightarrow$32 & 68$\rightarrow$52 & 100$\rightarrow$100 \\
% \bottomrule
% \end{tabular}%
% }
% \begin{tablenotes}[flushleft]
% \scriptsize
% \item[] \textbf{Note:} Format is \texttt{no aug$\rightarrow$aug}, indicating the complete disclosure rates before and after applying a privacy-aware prompt. E.g., ``100$\rightarrow$84'' means initially 100\% of sensitive information was disclosed, which reduced to 84\% after augmentation. Lower values indicate better performance. SSN: Social Security Number; Pwd: Phone Password; Setting: Setting of Conversation.
% \end{tablenotes}
% \end{table}


% 添加颜色2
% \begin{table}[!htbp]
% \centering
% \caption{Complete disclosure rate analysis: direct and inference privacy leakage (\%), lower is better.}
% \label{tab:complete_leakage_rate_privacy-leakage}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l|cc|cc|cc|cc|cc|cc|cc|cc|cc}
% \toprule
% \multirow{3}{*}{\textbf{Model}} & \multicolumn{12}{c|}{\textbf{Direct privacy leakage}} & \multicolumn{6}{c}{\textbf{Inference leakage}} \\
% \cmidrule(lr){2-13} \cmidrule(lr){14-19}
%  & \multicolumn{2}{c|}{\textbf{Bank Account}} & \multicolumn{2}{c|}{\textbf{Driver License}} & \multicolumn{2}{c|}{\textbf{Phone Number}} & \multicolumn{2}{c|}{\textbf{Pwd}} & \multicolumn{2}{c|}{\textbf{SSN}} & \multicolumn{2}{c|}{\textbf{Address}} & \multicolumn{2}{c|}{\textbf{Age}} & \multicolumn{2}{c|}{\textbf{Ethnicity}} & \multicolumn{2}{c}{\textbf{Setting}} \\
%  & \textbf{\footnotesize\centering no aug} & \textbf{\footnotesize\centering aug} & \textbf{\footnotesize\centering no aug} & \textbf{\footnotesize\centering aug} & \textbf{\footnotesize\centering no aug} & \textbf{\footnotesize\centering aug} & \textbf{\footnotesize\centering no aug} & \textbf{\footnotesize\centering aug} & \textbf{\footnotesize\centering no aug} & \textbf{\footnotesize\centering aug} & \textbf{\footnotesize\centering no aug} & \textbf{\footnotesize\centering aug} & \textbf{\footnotesize\centering no aug} & \textbf{\footnotesize\centering aug} & \textbf{\footnotesize\centering no aug} & \textbf{\footnotesize\centering aug} & \textbf{\footnotesize\centering no aug} & \textbf{\footnotesize\centering aug} \\
% \midrule
% \multicolumn{19}{c}{\textbf{Open-source Models}} \\
% \midrule
% \cellcolor{gray!10}Qwen2-Audio & \cellcolor{gray!10}100 & \cellcolor{gray!10}84 & \cellcolor{gray!10}99 & \cellcolor{gray!10}87 & \cellcolor{gray!10}100 & \cellcolor{gray!10}92 & \cellcolor{gray!10}96 & \cellcolor{gray!10}51 & \cellcolor{gray!10}100 & \cellcolor{gray!10}95 & \cellcolor{gray!10}100 & \cellcolor{gray!10}95 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 \\
% SALMONN & 49 & 3 & 43 & 2 & 36 & 9 & 27 & 1 & 34 & 1 & 70 & 0 & 3 & 0 & 67 & 87 & 100 & 75 \\
% \cellcolor{gray!10}MiniCPM-o 2.6 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 & \cellcolor{gray!10}94 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 \\
% UltraVox & 0 & 0 & 0 & 0 & 82 & 0 & 30 & 0 & 0 & 0 & 50 & 0 & 99 & 94 & 76 & 83 & 100 & 100 \\
% \midrule
% \multicolumn{19}{c}{\textbf{Closed-source Models}} \\
% \midrule
% \cellcolor{gray!10}Gemini-1.5 Pro & \cellcolor{gray!10}77 & \cellcolor{gray!10}0 & \cellcolor{gray!10}97 & \cellcolor{gray!10}0 & \cellcolor{gray!10}100 & \cellcolor{gray!10}0 & \cellcolor{gray!10}76 & \cellcolor{gray!10}0 & \cellcolor{gray!10}0 & \cellcolor{gray!10}0 & \cellcolor{gray!10}100 & \cellcolor{gray!10}5 & \cellcolor{gray!10}84 & \cellcolor{gray!10}72 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 \\
% Gemini-2.5 Flash & 100 & 0 & 100 & 0 & 100 & 0 & 100 & 0 & 90 & 0 & 100 & 0 & 98 & 0 & 100 & 99 & 100 & 100 \\
% \cellcolor{gray!10}Gemini-2.5 Pro & \cellcolor{gray!10}100 & \cellcolor{gray!10}0 & \cellcolor{gray!10}100 & \cellcolor{gray!10}0 & \cellcolor{gray!10}0 & \cellcolor{gray!10}0 & \cellcolor{gray!10}100 & \cellcolor{gray!10}0 & \cellcolor{gray!10}0 & \cellcolor{gray!10}0 & \cellcolor{gray!10}100 & \cellcolor{gray!10}8 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 \\
% GPT-4o Audio & 0 & 0 & 0 & 0 & 30 & 1 & 0 & 0 & 0 & 0 & 12 & 1 & 98 & 78 & 83 & 69 & 100 & 96 \\
% \cellcolor{gray!10}GPT-4o Mini Audio & \cellcolor{gray!10}0 & \cellcolor{gray!10}0 & \cellcolor{gray!10}0 & \cellcolor{gray!10}0 & \cellcolor{gray!10}0 & \cellcolor{gray!10}0 & \cellcolor{gray!10}0 & \cellcolor{gray!10}0 & \cellcolor{gray!10}0 & \cellcolor{gray!10}0 & \cellcolor{gray!10}0 & \cellcolor{gray!10}0 & \cellcolor{gray!10}91 & \cellcolor{gray!10}32 & \cellcolor{gray!10}68 & \cellcolor{gray!10}52 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 \\
% \bottomrule
% \end{tabular}%
% }
% \begin{tablenotes}[flushleft]
% \scriptsize
% \item[] \textbf{Note:} "no aug" indicates the complete disclosure rates before applying a privacy-aware prompt, while "aug" shows rates after applying it. Lower values indicate better performance. SSN: Social Security Number; Pwd: Phone Password; Setting: Setting of Conversation.
% \end{tablenotes}
% \end{table}


% Average

% \begin{table}[!htbp]
% \centering
% \caption{Complete disclosure rate analysis: direct and inference privacy leakage (\%), lower is better.}
% \label{tab:complete_leakage_rate_privacy-leakage}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l|cc|cc|cc|cc|cc|cc|cc|cc|cc}
% \toprule
% \multirow{3}{*}{\textbf{Model}} & \multicolumn{12}{c|}{\textbf{Direct privacy leakage}} & \multicolumn{6}{c}{\textbf{Inference leakage}} \\
% \cmidrule(lr){2-13} \cmidrule(lr){14-19}
%  & \multicolumn{2}{c|}{\textbf{Bank Account}} & \multicolumn{2}{c|}{\textbf{Driver License}} & \multicolumn{2}{c|}{\textbf{Phone Number}} & \multicolumn{2}{c|}{\textbf{Pwd}} & \multicolumn{2}{c|}{\textbf{SSN}} & \multicolumn{2}{c|}{\textbf{Address}} & \multicolumn{2}{c|}{\textbf{Age}} & \multicolumn{2}{c|}{\textbf{Ethnicity}} & \multicolumn{2}{c}{\textbf{Setting}} \\
%  & \textbf{\footnotesize\centering no aug} & \textbf{\footnotesize\centering aug} & \textbf{\footnotesize\centering no aug} & \textbf{\footnotesize\centering aug} & \textbf{\footnotesize\centering no aug} & \textbf{\footnotesize\centering aug} & \textbf{\footnotesize\centering no aug} & \textbf{\footnotesize\centering aug} & \textbf{\footnotesize\centering no aug} & \textbf{\footnotesize\centering aug} & \textbf{\footnotesize\centering no aug} & \textbf{\footnotesize\centering aug} & \textbf{\footnotesize\centering no aug} & \textbf{\footnotesize\centering aug} & \textbf{\footnotesize\centering no aug} & \textbf{\footnotesize\centering aug} & \textbf{\footnotesize\centering no aug} & \textbf{\footnotesize\centering aug} \\
% \midrule
% \multicolumn{19}{c}{\textbf{Open-source Models}} \\
% \midrule
% \cellcolor{gray!10}Qwen2-Audio & \cellcolor{gray!10}100 & \cellcolor{gray!10}84 & \cellcolor{gray!10}99 & \cellcolor{gray!10}87 & \cellcolor{gray!10}100 & \cellcolor{gray!10}92 & \cellcolor{gray!10}96 & \cellcolor{gray!10}51 & \cellcolor{gray!10}100 & \cellcolor{gray!10}95 & \cellcolor{gray!10}100 & \cellcolor{gray!10}95 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 \\
% SALMONN & 49 & 3 & 43 & 2 & 36 & 9 & 27 & 1 & 34 & 1 & 70 & 0 & 3 & 0 & 67 & 87 & 100 & 75 \\
% \cellcolor{gray!10}MiniCPM-o 2.6 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 & \cellcolor{gray!10}94 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 \\
% UltraVox & 0 & 0 & 0 & 0 & 82 & 0 & 30 & 0 & 0 & 0 & 50 & 0 & 99 & 94 & 76 & 83 & 100 & 100 \\
% \midrule
% \multicolumn{19}{c}{\textbf{Closed-source Models}} \\
% \midrule
% \cellcolor{gray!10}Gemini-1.5 Pro & \cellcolor{gray!10}77 & \cellcolor{gray!10}0 & \cellcolor{gray!10}97 & \cellcolor{gray!10}0 & \cellcolor{gray!10}100 & \cellcolor{gray!10}0 & \cellcolor{gray!10}76 & \cellcolor{gray!10}0 & \cellcolor{gray!10}0 & \cellcolor{gray!10}0 & \cellcolor{gray!10}100 & \cellcolor{gray!10}5 & \cellcolor{gray!10}84 & \cellcolor{gray!10}72 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 \\
% Gemini-2.5 Flash & 100 & 0 & 100 & 0 & 100 & 0 & 100 & 0 & 90 & 0 & 100 & 0 & 98 & 0 & 100 & 99 & 100 & 100 \\
% \cellcolor{gray!10}Gemini-2.5 Pro & \cellcolor{gray!10}100 & \cellcolor{gray!10}0 & \cellcolor{gray!10}100 & \cellcolor{gray!10}0 & \cellcolor{gray!10}0 & \cellcolor{gray!10}0 & \cellcolor{gray!10}100 & \cellcolor{gray!10}0 & \cellcolor{gray!10}0 & \cellcolor{gray!10}0 & \cellcolor{gray!10}100 & \cellcolor{gray!10}8 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 \\
% GPT-4o Audio & 0 & 0 & 0 & 0 & 30 & 1 & 0 & 0 & 0 & 0 & 12 & 1 & 98 & 78 & 83 & 69 & 100 & 96 \\
% \cellcolor{gray!10}GPT-4o Mini Audio & \cellcolor{gray!10}0 & \cellcolor{gray!10}0 & \cellcolor{gray!10}0 & \cellcolor{gray!10}0 & \cellcolor{gray!10}0 & \cellcolor{gray!10}0 & \cellcolor{gray!10}0 & \cellcolor{gray!10}0 & \cellcolor{gray!10}0 & \cellcolor{gray!10}0 & \cellcolor{gray!10}0 & \cellcolor{gray!10}0 & \cellcolor{gray!10}91 & \cellcolor{gray!10}32 & \cellcolor{gray!10}68 & \cellcolor{gray!10}52 & \cellcolor{gray!10}100 & \cellcolor{gray!10}100 \\
% \hline
% Average & 58.4 & 20.8 & 59.9 & 21.0 & 60.9 & 22.4 & 58.8 & 16.2 & 36.0 & 21.8 & 70.2 & 23.2 & 85.9 & 64.0 & 88.2 & 87.8 & 100.0 & 96.8 \\
% \bottomrule
% \end{tabular}%
% }
% \begin{tablenotes}[flushleft]
% \scriptsize
% \item[] \textbf{Note:} "no aug" indicates the complete disclosure rates before applying a privacy-aware prompt, while "aug" shows rates after applying it. Lower values indicate better performance. SSN: Social Security Number; Pwd: Phone Password; Setting: Setting of Conversation.
% \end{tablenotes}
% \end{table}

% final
% \begin{table}[!htbp]
% \centering
% \caption{Complete disclosure rate analysis: direct and inference privacy leakage (\%), lower is better.}
% \label{tab:complete_leakage_rate_privacy-leakage}
% \renewcommand{\arraystretch}{1.5} % 增加行高，原来没有设置，
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l|cc|cc|cc|cc|cc|cc|cc|cc|cc}
% \toprule
% \multirow{3}{*}{\textbf{Model}} & \multicolumn{12}{c|}{\textbf{Direct privacy leakage}} & \multicolumn{6}{c}{\textbf{Inference leakage}} \\
% \cmidrule(lr){2-13} \cmidrule(lr){14-19}
%  & \multicolumn{2}{c|}{\textbf{Bank Account}} & \multicolumn{2}{c|}{\textbf{Driver License}} & \multicolumn{2}{c|}{\textbf{Phone Number}} & \multicolumn{2}{c|}{\textbf{Pwd}} & \multicolumn{2}{c|}{\textbf{SSN}} & \multicolumn{2}{c|}{\textbf{Address}} & \multicolumn{2}{c|}{\textbf{Age}} & \multicolumn{2}{c|}{\textbf{Ethnicity}} & \multicolumn{2}{c}{\textbf{Setting}} \\
%  & \textbf{\footnotesize\centering no aug} & \textbf{\footnotesize\centering aug} & \textbf{\footnotesize\centering no aug} & \textbf{\footnotesize\centering aug} & \textbf{\footnotesize\centering no aug} & \textbf{\footnotesize\centering aug} & \textbf{\footnotesize\centering no aug} & \textbf{\footnotesize\centering aug} & \textbf{\footnotesize\centering no aug} & \textbf{\footnotesize\centering aug} & \textbf{\footnotesize\centering no aug} & \textbf{\footnotesize\centering aug} & \textbf{\footnotesize\centering no aug} & \textbf{\footnotesize\centering aug} & \textbf{\footnotesize\centering no aug} & \textbf{\footnotesize\centering aug} & \textbf{\footnotesize\centering no aug} & \textbf{\footnotesize\centering aug} \\
% \midrule
% \multicolumn{19}{c}{\textbf{Open-source Models}} \\
% \midrule
% \cellcolor{gray!10}Qwen2-Audio & \cellcolor{gray!10}100 $\textcolor{red}{\uparrow_{\scriptsize 41.6}}$ & \cellcolor{gray!10}84 $\textcolor{red}{\uparrow_{\scriptsize 63.2}}$ & \cellcolor{gray!10}99 $\textcolor{red}{\uparrow_{\scriptsize 39.1}}$ & \cellcolor{gray!10}87 $\textcolor{red}{\uparrow_{\scriptsize 66.0}}$ & \cellcolor{gray!10}100 $\textcolor{red}{\uparrow_{\scriptsize 39.1}}$ & \cellcolor{gray!10}92 $\textcolor{red}{\uparrow_{\scriptsize 69.6}}$ & \cellcolor{gray!10}96 $\textcolor{red}{\uparrow_{\scriptsize 37.2}}$ & \cellcolor{gray!10}51 $\textcolor{red}{\uparrow_{\scriptsize 34.8}}$ & \cellcolor{gray!10}100 $\textcolor{red}{\uparrow_{\scriptsize 64.0}}$ & \cellcolor{gray!10}95 $\textcolor{red}{\uparrow_{\scriptsize 73.2}}$ & \cellcolor{gray!10}100 $\textcolor{red}{\uparrow_{\scriptsize 29.8}}$ & \cellcolor{gray!10}95 $\textcolor{red}{\uparrow_{\scriptsize 71.8}}$ & \cellcolor{gray!10}100 $\textcolor{red}{\uparrow_{\scriptsize 14.1}}$ & \cellcolor{gray!10}100 $\textcolor{red}{\uparrow_{\scriptsize 36.0}}$ & \cellcolor{gray!10}100 $\textcolor{red}{\uparrow_{\scriptsize 11.8}}$ & \cellcolor{gray!10}100 $\textcolor{red}{\uparrow_{\scriptsize 12.2}}$ & \cellcolor{gray!10}100 $\textcolor{red}{\uparrow_{\scriptsize 0.0}}$ & \cellcolor{gray!10}100 $\textcolor{red}{\uparrow_{\scriptsize 3.2}}$ \\
% SALMONN & 49 $\textcolor{blue}{\downarrow_{\scriptsize 9.4}}$ & 3 $\textcolor{blue}{\downarrow_{\scriptsize 17.8}}$ & 43 $\textcolor{blue}{\downarrow_{\scriptsize 16.9}}$ & 2 $\textcolor{blue}{\downarrow_{\scriptsize 19.0}}$ & 36 $\textcolor{blue}{\downarrow_{\scriptsize 24.9}}$ & 9 $\textcolor{blue}{\downarrow_{\scriptsize 13.4}}$ & 27 $\textcolor{blue}{\downarrow_{\scriptsize 31.8}}$ & 1 $\textcolor{blue}{\downarrow_{\scriptsize 15.2}}$ & 34 $\textcolor{blue}{\downarrow_{\scriptsize 2.0}}$ & 1 $\textcolor{blue}{\downarrow_{\scriptsize 20.8}}$ & 70 $\textcolor{blue}{\downarrow_{\scriptsize 0.2}}$ & 0 $\textcolor{blue}{\downarrow_{\scriptsize 23.2}}$ & 3 $\textcolor{blue}{\downarrow_{\scriptsize 82.9}}$ & 0 $\textcolor{blue}{\downarrow_{\scriptsize 64.0}}$ & 67 $\textcolor{blue}{\downarrow_{\scriptsize 21.2}}$ & 87 $\textcolor{blue}{\downarrow_{\scriptsize 0.8}}$ & 100 $\textcolor{red}{\uparrow_{\scriptsize 0.0}}$ & 75 $\textcolor{blue}{\downarrow_{\scriptsize 21.8}}$ \\
% \cellcolor{gray!10}MiniCPM-o 2.6 & \cellcolor{gray!10}100 $\textcolor{red}{\uparrow_{\scriptsize 41.6}}$ & \cellcolor{gray!10}100 $\textcolor{red}{\uparrow_{\scriptsize 79.2}}$ & \cellcolor{gray!10}100 $\textcolor{red}{\uparrow_{\scriptsize 40.1}}$ & \cellcolor{gray!10}100 $\textcolor{red}{\uparrow_{\scriptsize 79.0}}$ & \cellcolor{gray!10}100 $\textcolor{red}{\uparrow_{\scriptsize 39.1}}$ & \cellcolor{gray!10}100 $\textcolor{red}{\uparrow_{\scriptsize 77.6}}$ & \cellcolor{gray!10}100 $\textcolor{red}{\uparrow_{\scriptsize 41.2}}$ & \cellcolor{gray!10}94 $\textcolor{red}{\uparrow_{\scriptsize 77.8}}$ & \cellcolor{gray!10}100 $\textcolor{red}{\uparrow_{\scriptsize 64.0}}$ & \cellcolor{gray!10}100 $\textcolor{red}{\uparrow_{\scriptsize 78.2}}$ & \cellcolor{gray!10}100 $\textcolor{red}{\uparrow_{\scriptsize 29.8}}$ & \cellcolor{gray!10}100 $\textcolor{red}{\uparrow_{\scriptsize 76.8}}$ & \cellcolor{gray!10}100 $\textcolor{red}{\uparrow_{\scriptsize 14.1}}$ & \cellcolor{gray!10}100 $\textcolor{red}{\uparrow_{\scriptsize 36.0}}$ & \cellcolor{gray!10}100 $\textcolor{red}{\uparrow_{\scriptsize 11.8}}$ & \cellcolor{gray!10}100 $\textcolor{red}{\uparrow_{\scriptsize 12.2}}$ & \cellcolor{gray!10}100 $\textcolor{red}{\uparrow_{\scriptsize 0.0}}$ & \cellcolor{gray!10}100 $\textcolor{red}{\uparrow_{\scriptsize 3.2}}$ \\
% UltraVox & 0 $\textcolor{blue}{\downarrow_{\scriptsize 58.4}}$ & 0 $\textcolor{blue}{\downarrow_{\scriptsize 20.8}}$ & 0 $\textcolor{blue}{\downarrow_{\scriptsize 59.9}}$ & 0 $\textcolor{blue}{\downarrow_{\scriptsize 21.0}}$ & 82 $\textcolor{red}{\uparrow_{\scriptsize 21.1}}$ & 0 $\textcolor{blue}{\downarrow_{\scriptsize 22.4}}$ & 30 $\textcolor{blue}{\downarrow_{\scriptsize 28.8}}$ & 0 $\textcolor{blue}{\downarrow_{\scriptsize 16.2}}$ & 0 $\textcolor{blue}{\downarrow_{\scriptsize 36.0}}$ & 0 $\textcolor{blue}{\downarrow_{\scriptsize 21.8}}$ & 50 $\textcolor{blue}{\downarrow_{\scriptsize 20.2}}$ & 0 $\textcolor{blue}{\downarrow_{\scriptsize 23.2}}$ & 99 $\textcolor{red}{\uparrow_{\scriptsize 13.1}}$ & 94 $\textcolor{red}{\uparrow_{\scriptsize 30.0}}$ & 76 $\textcolor{blue}{\downarrow_{\scriptsize 12.2}}$ & 83 $\textcolor{blue}{\downarrow_{\scriptsize 4.8}}$ & 100 $\textcolor{red}{\uparrow_{\scriptsize 0.0}}$ & 100 $\textcolor{red}{\uparrow_{\scriptsize 3.2}}$ \\
% \midrule
% \multicolumn{19}{c}{\textbf{Closed-source Models}} \\
% \midrule
% \cellcolor{gray!10}Gemini-1.5 Pro & \cellcolor{gray!10}77 $\textcolor{red}{\uparrow_{\scriptsize 18.6}}$ & \cellcolor{gray!10}0 $\textcolor{blue}{\downarrow_{\scriptsize 20.8}}$ & \cellcolor{gray!10}97 $\textcolor{red}{\uparrow_{\scriptsize 37.1}}$ & \cellcolor{gray!10}0 $\textcolor{blue}{\downarrow_{\scriptsize 21.0}}$ & \cellcolor{gray!10}100 $\textcolor{red}{\uparrow_{\scriptsize 39.1}}$ & \cellcolor{gray!10}0 $\textcolor{blue}{\downarrow_{\scriptsize 22.4}}$ & \cellcolor{gray!10}76 $\textcolor{red}{\uparrow_{\scriptsize 17.2}}$ & \cellcolor{gray!10}0 $\textcolor{blue}{\downarrow_{\scriptsize 16.2}}$ & \cellcolor{gray!10}0 $\textcolor{blue}{\downarrow_{\scriptsize 36.0}}$ & \cellcolor{gray!10}0 $\textcolor{blue}{\downarrow_{\scriptsize 21.8}}$ & \cellcolor{gray!10}100 $\textcolor{red}{\uparrow_{\scriptsize 29.8}}$ & \cellcolor{gray!10}5 $\textcolor{blue}{\downarrow_{\scriptsize 18.2}}$ & \cellcolor{gray!10}84 $\textcolor{blue}{\downarrow_{\scriptsize 1.9}}$ & \cellcolor{gray!10}72 $\textcolor{red}{\uparrow_{\scriptsize 8.0}}$ & \cellcolor{gray!10}100 $\textcolor{red}{\uparrow_{\scriptsize 11.8}}$ & \cellcolor{gray!10}100 $\textcolor{red}{\uparrow_{\scriptsize 12.2}}$ & \cellcolor{gray!10}100 $\textcolor{red}{\uparrow_{\scriptsize 0.0}}$ & \cellcolor{gray!10}100 $\textcolor{red}{\uparrow_{\scriptsize 3.2}}$ \\
% Gemini-2.5 Flash & 100 $\textcolor{red}{\uparrow_{\scriptsize 41.6}}$ & 0 $\textcolor{blue}{\downarrow_{\scriptsize 20.8}}$ & 100 $\textcolor{red}{\uparrow_{\scriptsize 40.1}}$ & 0 $\textcolor{blue}{\downarrow_{\scriptsize 21.0}}$ & 100 $\textcolor{red}{\uparrow_{\scriptsize 39.1}}$ & 0 $\textcolor{blue}{\downarrow_{\scriptsize 22.4}}$ & 100 $\textcolor{red}{\uparrow_{\scriptsize 41.2}}$ & 0 $\textcolor{blue}{\downarrow_{\scriptsize 16.2}}$ & 90 $\textcolor{red}{\uparrow_{\scriptsize 54.0}}$ & 0 $\textcolor{blue}{\downarrow_{\scriptsize 21.8}}$ & 100 $\textcolor{red}{\uparrow_{\scriptsize 29.8}}$ & 0 $\textcolor{blue}{\downarrow_{\scriptsize 23.2}}$ & 98 $\textcolor{red}{\uparrow_{\scriptsize 12.1}}$ & 0 $\textcolor{blue}{\downarrow_{\scriptsize 64.0}}$ & 100 $\textcolor{red}{\uparrow_{\scriptsize 11.8}}$ & 99 $\textcolor{red}{\uparrow_{\scriptsize 11.2}}$ & 100 $\textcolor{red}{\uparrow_{\scriptsize 0.0}}$ & 100 $\textcolor{red}{\uparrow_{\scriptsize 3.2}}$ \\
% \cellcolor{gray!10}Gemini-2.5 Pro & \cellcolor{gray!10}100 $\textcolor{red}{\uparrow_{\scriptsize 41.6}}$ & \cellcolor{gray!10}0 $\textcolor{blue}{\downarrow_{\scriptsize 20.8}}$ & \cellcolor{gray!10}100 $\textcolor{red}{\uparrow_{\scriptsize 40.1}}$ & \cellcolor{gray!10}0 $\textcolor{blue}{\downarrow_{\scriptsize 21.0}}$ & \cellcolor{gray!10}0 $\textcolor{blue}{\downarrow_{\scriptsize 60.9}}$ & \cellcolor{gray!10}0 $\textcolor{blue}{\downarrow_{\scriptsize 22.4}}$ & \cellcolor{gray!10}100 $\textcolor{red}{\uparrow_{\scriptsize 41.2}}$ & \cellcolor{gray!10}0 $\textcolor{blue}{\downarrow_{\scriptsize 16.2}}$ & \cellcolor{gray!10}0 $\textcolor{blue}{\downarrow_{\scriptsize 36.0}}$ & \cellcolor{gray!10}0 $\textcolor{blue}{\downarrow_{\scriptsize 21.8}}$ & \cellcolor{gray!10}100 $\textcolor{red}{\uparrow_{\scriptsize 29.8}}$ & \cellcolor{gray!10}8 $\textcolor{blue}{\downarrow_{\scriptsize 15.2}}$ & \cellcolor{gray!10}100 $\textcolor{red}{\uparrow_{\scriptsize 14.1}}$ & \cellcolor{gray!10}100 $\textcolor{red}{\uparrow_{\scriptsize 36.0}}$ & \cellcolor{gray!10}100 $\textcolor{red}{\uparrow_{\scriptsize 11.8}}$ & \cellcolor{gray!10}100 $\textcolor{red}{\uparrow_{\scriptsize 12.2}}$ & \cellcolor{gray!10}100 $\textcolor{red}{\uparrow_{\scriptsize 0.0}}$ & \cellcolor{gray!10}100 $\textcolor{red}{\uparrow_{\scriptsize 3.2}}$ \\
% GPT-4o Audio & 0 $\textcolor{blue}{\downarrow_{\scriptsize 58.4}}$ & 0 $\textcolor{blue}{\downarrow_{\scriptsize 20.8}}$ & 0 $\textcolor{blue}{\downarrow_{\scriptsize 59.9}}$ & 0 $\textcolor{blue}{\downarrow_{\scriptsize 21.0}}$ & 30 $\textcolor{blue}{\downarrow_{\scriptsize 30.9}}$ & 1 $\textcolor{blue}{\downarrow_{\scriptsize 21.4}}$ & 0 $\textcolor{blue}{\downarrow_{\scriptsize 58.8}}$ & 0 $\textcolor{blue}{\downarrow_{\scriptsize 16.2}}$ & 0 $\textcolor{blue}{\downarrow_{\scriptsize 36.0}}$ & 0 $\textcolor{blue}{\downarrow_{\scriptsize 21.8}}$ & 12 $\textcolor{blue}{\downarrow_{\scriptsize 58.2}}$ & 1 $\textcolor{blue}{\downarrow_{\scriptsize 22.2}}$ & 98 $\textcolor{red}{\uparrow_{\scriptsize 12.1}}$ & 78 $\textcolor{red}{\uparrow_{\scriptsize 14.0}}$ & 83 $\textcolor{blue}{\downarrow_{\scriptsize 5.2}}$ & 69 $\textcolor{blue}{\downarrow_{\scriptsize 18.8}}$ & 100 $\textcolor{red}{\uparrow_{\scriptsize 0.0}}$ & 96 $\textcolor{blue}{\downarrow_{\scriptsize 0.8}}$ \\
% \cellcolor{gray!10}GPT-4o Mini Audio & \cellcolor{gray!10}0 $\textcolor{blue}{\downarrow_{\scriptsize 58.4}}$ & \cellcolor{gray!10}0 $\textcolor{blue}{\downarrow_{\scriptsize 20.8}}$ & \cellcolor{gray!10}0 $\textcolor{blue}{\downarrow_{\scriptsize 59.9}}$ & \cellcolor{gray!10}0 $\textcolor{blue}{\downarrow_{\scriptsize 21.0}}$ & \cellcolor{gray!10}0 $\textcolor{blue}{\downarrow_{\scriptsize 60.9}}$ & \cellcolor{gray!10}0 $\textcolor{blue}{\downarrow_{\scriptsize 22.4}}$ & \cellcolor{gray!10}0 $\textcolor{blue}{\downarrow_{\scriptsize 58.8}}$ & \cellcolor{gray!10}0 $\textcolor{blue}{\downarrow_{\scriptsize 16.2}}$ & \cellcolor{gray!10}0 $\textcolor{blue}{\downarrow_{\scriptsize 36.0}}$ & \cellcolor{gray!10}0 $\textcolor{blue}{\downarrow_{\scriptsize 21.8}}$ & \cellcolor{gray!10}0 $\textcolor{blue}{\downarrow_{\scriptsize 70.2}}$ & \cellcolor{gray!10}0 $\textcolor{blue}{\downarrow_{\scriptsize 23.2}}$ & \cellcolor{gray!10}91 $\textcolor{red}{\uparrow_{\scriptsize 5.1}}$ & \cellcolor{gray!10}32 $\textcolor{blue}{\downarrow_{\scriptsize 32.0}}$ & \cellcolor{gray!10}68 $\textcolor{blue}{\downarrow_{\scriptsize 20.2}}$ & \cellcolor{gray!10}52 $\textcolor{blue}{\downarrow_{\scriptsize 35.8}}$ & \cellcolor{gray!10}100 $\textcolor{red}{\uparrow_{\scriptsize 0.0}}$ & \cellcolor{gray!10}100 $\textcolor{red}{\uparrow_{\scriptsize 3.2}}$ \\
% \hline
% Average & 58.4 & 20.8 & 59.9 & 21.0 & 60.9 & 22.4 & 58.8 & 16.2 & 36.0 & 21.8 & 70.2 & 23.2 & 85.9 & 64.0 & 88.2 & 87.8 & 100.0 & 96.8 \\
% \bottomrule
% \end{tabular}%
% }
% \begin{tablenotes}[flushleft]
% \scriptsize
% \item[] \textbf{Note:} "no aug" indicates the complete disclosure rates before applying a privacy-aware prompt, while "aug" shows rates after applying it. Lower values indicate better performance. Red arrows ($\textcolor{red}{\uparrow}$) indicate worse performance (higher leakage) than average; blue arrows ($\textcolor{blue}{\downarrow}$) indicate better performance (lower leakage) than average. SSN: Social Security Number; Pwd: Phone Password; Setting: Setting of Conversation.
% \end{tablenotes}
% \end{table}


% with 行高
% \begin{table}[!htbp]
% \centering
% \caption{Complete disclosure rate analysis: direct and inference privacy leakage (\%), lower is better.}
% \label{tab:complete_leakage_rate_privacy-leakage}
% \renewcommand{\arraystretch}{1.5} % 保持增加的行高
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l|cc|cc|cc|cc|cc|cc|cc|cc|cc}
% \toprule
% \multirow{3}{*}{\large\textbf{Model}} & \multicolumn{12}{c|}{\large\textbf{Direct privacy leakage}} & \multicolumn{6}{c}{\large\textbf{Inference leakage}} \\
% \cmidrule(lr){2-13} \cmidrule(lr){14-19}
%  & \multicolumn{2}{c|}{\textbf{Bank Account}} & \multicolumn{2}{c|}{\textbf{Driver License}} & \multicolumn{2}{c|}{\textbf{Phone Number}} & \multicolumn{2}{c|}{\textbf{Pwd}} & \multicolumn{2}{c|}{\textbf{SSN}} & \multicolumn{2}{c|}{\textbf{Address}} & \multicolumn{2}{c|}{\textbf{Age}} & \multicolumn{2}{c|}{\textbf{Ethnicity}} & \multicolumn{2}{c}{\textbf{Setting}} \\
%  & \textbf{\small\centering no aug} & \textbf{\small\centering aug} & \textbf{\small\centering no aug} & \textbf{\small\centering aug} & \textbf{\small\centering no aug} & \textbf{\small\centering aug} & \textbf{\small\centering no aug} & \textbf{\small\centering aug} & \textbf{\small\centering no aug} & \textbf{\small\centering aug} & \textbf{\small\centering no aug} & \textbf{\small\centering aug} & \textbf{\small\centering no aug} & \textbf{\small\centering aug} & \textbf{\small\centering no aug} & \textbf{\small\centering aug} & \textbf{\small\centering no aug} & \textbf{\small\centering aug} \\
% \midrule
% \multicolumn{19}{c}{\large\textbf{Open-source Models}} \\
% \midrule
% \cellcolor{gray!10}\normalsize Qwen2-Audio & \cellcolor{gray!10}\normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 41.6}}$ & \cellcolor{gray!10}\normalsize 84 $\textcolor{red}{\uparrow_{\scriptsize 63.2}}$ & \cellcolor{gray!10}\normalsize 99 $\textcolor{red}{\uparrow_{\scriptsize 39.1}}$ & \cellcolor{gray!10}\normalsize 87 $\textcolor{red}{\uparrow_{\scriptsize 66.0}}$ & \cellcolor{gray!10}\normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 39.1}}$ & \cellcolor{gray!10}\normalsize 92 $\textcolor{red}{\uparrow_{\scriptsize 69.6}}$ & \cellcolor{gray!10}\normalsize 96 $\textcolor{red}{\uparrow_{\scriptsize 37.2}}$ & \cellcolor{gray!10}\normalsize 51 $\textcolor{red}{\uparrow_{\scriptsize 34.8}}$ & \cellcolor{gray!10}\normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 64.0}}$ & \cellcolor{gray!10}\normalsize 95 $\textcolor{red}{\uparrow_{\scriptsize 73.2}}$ & \cellcolor{gray!10}\normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 29.8}}$ & \cellcolor{gray!10}\normalsize 95 $\textcolor{red}{\uparrow_{\scriptsize 71.8}}$ & \cellcolor{gray!10}\normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 14.1}}$ & \cellcolor{gray!10}\normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 36.0}}$ & \cellcolor{gray!10}\normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 11.8}}$ & \cellcolor{gray!10}\normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 12.2}}$ & \cellcolor{gray!10}\normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 0.0}}$ & \cellcolor{gray!10}\normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 3.2}}$ \\
% \normalsize SALMONN & \normalsize 49 $\textcolor{blue}{\downarrow_{\scriptsize 9.4}}$ & \normalsize 3 $\textcolor{blue}{\downarrow_{\scriptsize 17.8}}$ & \normalsize 43 $\textcolor{blue}{\downarrow_{\scriptsize 16.9}}$ & \normalsize 2 $\textcolor{blue}{\downarrow_{\scriptsize 19.0}}$ & \normalsize 36 $\textcolor{blue}{\downarrow_{\scriptsize 24.9}}$ & \normalsize 9 $\textcolor{blue}{\downarrow_{\scriptsize 13.4}}$ & \normalsize 27 $\textcolor{blue}{\downarrow_{\scriptsize 31.8}}$ & \normalsize 1 $\textcolor{blue}{\downarrow_{\scriptsize 15.2}}$ & \normalsize 34 $\textcolor{blue}{\downarrow_{\scriptsize 2.0}}$ & \normalsize 1 $\textcolor{blue}{\downarrow_{\scriptsize 20.8}}$ & \normalsize 70 $\textcolor{blue}{\downarrow_{\scriptsize 0.2}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 23.2}}$ & \normalsize 3 $\textcolor{blue}{\downarrow_{\scriptsize 82.9}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 64.0}}$ & \normalsize 67 $\textcolor{blue}{\downarrow_{\scriptsize 21.2}}$ & \normalsize 87 $\textcolor{blue}{\downarrow_{\scriptsize 0.8}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 0.0}}$ & \normalsize 75 $\textcolor{blue}{\downarrow_{\scriptsize 21.8}}$ \\
% \cellcolor{gray!10}\normalsize MiniCPM-o 2.6 & \cellcolor{gray!10}\normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 41.6}}$ & \cellcolor{gray!10}\normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 79.2}}$ & \cellcolor{gray!10}\normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 40.1}}$ & \cellcolor{gray!10}\normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 79.0}}$ & \cellcolor{gray!10}\normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 39.1}}$ & \cellcolor{gray!10}\normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 77.6}}$ & \cellcolor{gray!10}\normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 41.2}}$ & \cellcolor{gray!10}\normalsize 94 $\textcolor{red}{\uparrow_{\scriptsize 77.8}}$ & \cellcolor{gray!10}\normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 64.0}}$ & \cellcolor{gray!10}\normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 78.2}}$ & \cellcolor{gray!10}\normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 29.8}}$ & \cellcolor{gray!10}\normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 76.8}}$ & \cellcolor{gray!10}\normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 14.1}}$ & \cellcolor{gray!10}\normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 36.0}}$ & \cellcolor{gray!10}\normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 11.8}}$ & \cellcolor{gray!10}\normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 12.2}}$ & \cellcolor{gray!10}\normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 0.0}}$ & \cellcolor{gray!10}\normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 3.2}}$ \\
% \normalsize UltraVox & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 58.4}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 20.8}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 59.9}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 21.0}}$ & \normalsize 82 $\textcolor{red}{\uparrow_{\scriptsize 21.1}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 22.4}}$ & \normalsize 30 $\textcolor{blue}{\downarrow_{\scriptsize 28.8}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 16.2}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 36.0}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 21.8}}$ & \normalsize 50 $\textcolor{blue}{\downarrow_{\scriptsize 20.2}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 23.2}}$ & \normalsize 99 $\textcolor{red}{\uparrow_{\scriptsize 13.1}}$ & \normalsize 94 $\textcolor{red}{\uparrow_{\scriptsize 30.0}}$ & \normalsize 76 $\textcolor{blue}{\downarrow_{\scriptsize 12.2}}$ & \normalsize 83 $\textcolor{blue}{\downarrow_{\scriptsize 4.8}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 0.0}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 3.2}}$ \\
% \midrule
% \multicolumn{19}{c}{\large\textbf{Closed-source Models}} \\
% \midrule
% \cellcolor{gray!10}\normalsize Gemini-1.5 Pro & \cellcolor{gray!10}\normalsize 77 $\textcolor{red}{\uparrow_{\scriptsize 18.6}}$ & \cellcolor{gray!10}\normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 20.8}}$ & \cellcolor{gray!10}\normalsize 97 $\textcolor{red}{\uparrow_{\scriptsize 37.1}}$ & \cellcolor{gray!10}\normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 21.0}}$ & \cellcolor{gray!10}\normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 39.1}}$ & \cellcolor{gray!10}\normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 22.4}}$ & \cellcolor{gray!10}\normalsize 76 $\textcolor{red}{\uparrow_{\scriptsize 17.2}}$ & \cellcolor{gray!10}\normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 16.2}}$ & \cellcolor{gray!10}\normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 36.0}}$ & \cellcolor{gray!10}\normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 21.8}}$ & \cellcolor{gray!10}\normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 29.8}}$ & \cellcolor{gray!10}\normalsize 5 $\textcolor{blue}{\downarrow_{\scriptsize 18.2}}$ & \cellcolor{gray!10}\normalsize 84 $\textcolor{blue}{\downarrow_{\scriptsize 1.9}}$ & \cellcolor{gray!10}\normalsize 72 $\textcolor{red}{\uparrow_{\scriptsize 8.0}}$ & \cellcolor{gray!10}\normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 11.8}}$ & \cellcolor{gray!10}\normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 12.2}}$ & \cellcolor{gray!10}\normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 0.0}}$ & \cellcolor{gray!10}\normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 3.2}}$ \\
% \normalsize Gemini-2.5 Flash & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 41.6}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 20.8}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 40.1}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 21.0}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 39.1}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 22.4}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 41.2}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 16.2}}$ & \normalsize 90 $\textcolor{red}{\uparrow_{\scriptsize 54.0}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 21.8}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 29.8}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 23.2}}$ & \normalsize 98 $\textcolor{red}{\uparrow_{\scriptsize 12.1}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 64.0}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 11.8}}$ & \normalsize 99 $\textcolor{red}{\uparrow_{\scriptsize 11.2}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 0.0}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 3.2}}$ \\
% \cellcolor{gray!10}\normalsize Gemini-2.5 Pro & \cellcolor{gray!10}\normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 41.6}}$ & \cellcolor{gray!10}\normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 20.8}}$ & \cellcolor{gray!10}\normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 40.1}}$ & \cellcolor{gray!10}\normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 21.0}}$ & \cellcolor{gray!10}\normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 60.9}}$ & \cellcolor{gray!10}\normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 22.4}}$ & \cellcolor{gray!10}\normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 41.2}}$ & \cellcolor{gray!10}\normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 16.2}}$ & \cellcolor{gray!10}\normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 36.0}}$ & \cellcolor{gray!10}\normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 21.8}}$ & \cellcolor{gray!10}\normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 29.8}}$ & \cellcolor{gray!10}\normalsize 8 $\textcolor{blue}{\downarrow_{\scriptsize 15.2}}$ & \cellcolor{gray!10}\normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 14.1}}$ & \cellcolor{gray!10}\normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 36.0}}$ & \cellcolor{gray!10}\normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 11.8}}$ & \cellcolor{gray!10}\normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 12.2}}$ & \cellcolor{gray!10}\normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 0.0}}$ & \cellcolor{gray!10}\normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 3.2}}$ \\
% \normalsize GPT-4o Audio & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 58.4}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 20.8}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 59.9}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 21.0}}$ & \normalsize 30 $\textcolor{blue}{\downarrow_{\scriptsize 30.9}}$ & \normalsize 1 $\textcolor{blue}{\downarrow_{\scriptsize 21.4}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 58.8}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 16.2}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 36.0}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 21.8}}$ & \normalsize 12 $\textcolor{blue}{\downarrow_{\scriptsize 58.2}}$ & \normalsize 1 $\textcolor{blue}{\downarrow_{\scriptsize 22.2}}$ & \normalsize 98 $\textcolor{red}{\uparrow_{\scriptsize 12.1}}$ & \normalsize 78 $\textcolor{red}{\uparrow_{\scriptsize 14.0}}$ & \normalsize 83 $\textcolor{blue}{\downarrow_{\scriptsize 5.2}}$ & \normalsize 69 $\textcolor{blue}{\downarrow_{\scriptsize 18.8}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 0.0}}$ & \normalsize 96 $\textcolor{blue}{\downarrow_{\scriptsize 0.8}}$ \\
% \cellcolor{gray!10}\normalsize GPT-4o Mini Audio & \cellcolor{gray!10}\normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 58.4}}$ & \cellcolor{gray!10}\normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 20.8}}$ & \cellcolor{gray!10}\normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 59.9}}$ & \cellcolor{gray!10}\normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 21.0}}$ & \cellcolor{gray!10}\normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 60.9}}$ & \cellcolor{gray!10}\normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 22.4}}$ & \cellcolor{gray!10}\normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 58.8}}$ & \cellcolor{gray!10}\normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 16.2}}$ & \cellcolor{gray!10}\normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 36.0}}$ & \cellcolor{gray!10}\normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 21.8}}$ & \cellcolor{gray!10}\normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 70.2}}$ & \cellcolor{gray!10}\normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 23.2}}$ & \cellcolor{gray!10}\normalsize 91 $\textcolor{red}{\uparrow_{\scriptsize 5.1}}$ & \cellcolor{gray!10}\normalsize 32 $\textcolor{blue}{\downarrow_{\scriptsize 32.0}}$ & \cellcolor{gray!10}\normalsize 68 $\textcolor{blue}{\downarrow_{\scriptsize 20.2}}$ & \cellcolor{gray!10}\normalsize 52 $\textcolor{blue}{\downarrow_{\scriptsize 35.8}}$ & \cellcolor{gray!10}\normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 0.0}}$ & \cellcolor{gray!10}\normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 3.2}}$ \\
% \hline
% \normalsize Average & \normalsize 58.4 & \normalsize 20.8 & \normalsize 59.9 & \normalsize 21.0 & \normalsize 60.9 & \normalsize 22.4 & \normalsize 58.8 & \normalsize 16.2 & \normalsize 36.0 & \normalsize 21.8 & \normalsize 70.2 & \normalsize 23.2 & \normalsize 85.9 & \normalsize 64.0 & \normalsize 88.2 & \normalsize 87.8 & \normalsize 100.0 & \normalsize 96.8 \\
% \bottomrule
% \end{tabular}%
% }
% \begin{tablenotes}[flushleft]
% \scriptsize
% \item[] \textbf{Note:} "no aug" indicates the complete disclosure rates before applying a privacy-aware prompt, while "aug" shows rates after applying it. Lower values indicate better performance. Red arrows ($\textcolor{red}{\uparrow}$) indicate worse performance (higher leakage) than average; blue arrows ($\textcolor{blue}{\downarrow}$) indicate better performance (lower leakage) than average. SSN: Social Security Number; Pwd: Phone Password; Setting: Setting of Conversation.
% \end{tablenotes}
% \end{table}

% 边框修改

% \begin{table}[!htbp]
% \centering
% \caption{Complete disclosure rate analysis: direct and inference privacy leakage (\%), lower is better.}
% \label{tab:complete_leakage_rate_privacy-leakage}
% \renewcommand{\arraystretch}{1.5} % 保持增加的行高
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l|cc|cc|cc|cc|cc|cc|cc|cc|cc}
% \toprule
% \multirow{3}{*}{\large\textbf{Model}} & \multicolumn{12}{c|}{\large\textbf{Direct privacy leakage}} & \multicolumn{6}{c}{\large\textbf{Inference leakage}} \\
% \cmidrule(lr){2-13} \cmidrule(lr){14-19}
%  & \multicolumn{2}{c|}{\textbf{Bank Account}} & \multicolumn{2}{c|}{\textbf{Driver License}} & \multicolumn{2}{c|}{\textbf{Phone Number}} & \multicolumn{2}{c|}{\textbf{Pwd}} & \multicolumn{2}{c|}{\textbf{SSN}} & \multicolumn{2}{c|}{\textbf{Address}} & \multicolumn{2}{c|}{\textbf{Age}} & \multicolumn{2}{c|}{\textbf{Ethnicity}} & \multicolumn{2}{c}{\textbf{Setting}} \\
%  & \textbf{\small\centering no aug} & \textbf{\small\centering aug} & \textbf{\small\centering no aug} & \textbf{\small\centering aug} & \textbf{\small\centering no aug} & \textbf{\small\centering aug} & \textbf{\small\centering no aug} & \textbf{\small\centering aug} & \textbf{\small\centering no aug} & \textbf{\small\centering aug} & \textbf{\small\centering no aug} & \textbf{\small\centering aug} & \textbf{\small\centering no aug} & \textbf{\small\centering aug} & \textbf{\small\centering no aug} & \textbf{\small\centering aug} & \textbf{\small\centering no aug} & \textbf{\small\centering aug} \\
% \midrule
% \multicolumn{19}{c}{\large\textbf{Open-source Models}} \\
% \midrule
% \rowcolor{gray!10} \normalsize Qwen2-Audio & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 41.6}}$ & \normalsize 84 $\textcolor{red}{\uparrow_{\scriptsize 63.2}}$ & \normalsize 99 $\textcolor{red}{\uparrow_{\scriptsize 39.1}}$ & \normalsize 87 $\textcolor{red}{\uparrow_{\scriptsize 66.0}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 39.1}}$ & \normalsize 92 $\textcolor{red}{\uparrow_{\scriptsize 69.6}}$ & \normalsize 96 $\textcolor{red}{\uparrow_{\scriptsize 37.2}}$ & \normalsize 51 $\textcolor{red}{\uparrow_{\scriptsize 34.8}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 64.0}}$ & \normalsize 95 $\textcolor{red}{\uparrow_{\scriptsize 73.2}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 29.8}}$ & \normalsize 95 $\textcolor{red}{\uparrow_{\scriptsize 71.8}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 14.1}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 36.0}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 11.8}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 12.2}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 0.0}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 3.2}}$ \\
% \normalsize SALMONN & \normalsize 49 $\textcolor{blue}{\downarrow_{\scriptsize 9.4}}$ & \normalsize 3 $\textcolor{blue}{\downarrow_{\scriptsize 17.8}}$ & \normalsize 43 $\textcolor{blue}{\downarrow_{\scriptsize 16.9}}$ & \normalsize 2 $\textcolor{blue}{\downarrow_{\scriptsize 19.0}}$ & \normalsize 36 $\textcolor{blue}{\downarrow_{\scriptsize 24.9}}$ & \normalsize 9 $\textcolor{blue}{\downarrow_{\scriptsize 13.4}}$ & \normalsize 27 $\textcolor{blue}{\downarrow_{\scriptsize 31.8}}$ & \normalsize 1 $\textcolor{blue}{\downarrow_{\scriptsize 15.2}}$ & \normalsize 34 $\textcolor{blue}{\downarrow_{\scriptsize 2.0}}$ & \normalsize 1 $\textcolor{blue}{\downarrow_{\scriptsize 20.8}}$ & \normalsize 70 $\textcolor{blue}{\downarrow_{\scriptsize 0.2}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 23.2}}$ & \normalsize 3 $\textcolor{blue}{\downarrow_{\scriptsize 82.9}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 64.0}}$ & \normalsize 67 $\textcolor{blue}{\downarrow_{\scriptsize 21.2}}$ & \normalsize 87 $\textcolor{blue}{\downarrow_{\scriptsize 0.8}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 0.0}}$ & \normalsize 75 $\textcolor{blue}{\downarrow_{\scriptsize 21.8}}$ \\
% \rowcolor{gray!10} \normalsize MiniCPM-o 2.6 & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 41.6}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 79.2}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 40.1}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 79.0}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 39.1}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 77.6}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 41.2}}$ & \normalsize 94 $\textcolor{red}{\uparrow_{\scriptsize 77.8}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 64.0}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 78.2}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 29.8}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 76.8}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 14.1}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 36.0}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 11.8}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 12.2}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 0.0}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 3.2}}$ \\
% \normalsize UltraVox & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 58.4}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 20.8}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 59.9}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 21.0}}$ & \normalsize 82 $\textcolor{red}{\uparrow_{\scriptsize 21.1}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 22.4}}$ & \normalsize 30 $\textcolor{blue}{\downarrow_{\scriptsize 28.8}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 16.2}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 36.0}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 21.8}}$ & \normalsize 50 $\textcolor{blue}{\downarrow_{\scriptsize 20.2}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 23.2}}$ & \normalsize 99 $\textcolor{red}{\uparrow_{\scriptsize 13.1}}$ & \normalsize 94 $\textcolor{red}{\uparrow_{\scriptsize 30.0}}$ & \normalsize 76 $\textcolor{blue}{\downarrow_{\scriptsize 12.2}}$ & \normalsize 83 $\textcolor{blue}{\downarrow_{\scriptsize 4.8}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 0.0}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 3.2}}$ \\
% \midrule
% \multicolumn{19}{c}{\large\textbf{Closed-source Models}} \\
% \midrule
% \rowcolor{gray!10} \normalsize Gemini-1.5 Pro & \normalsize 77 $\textcolor{red}{\uparrow_{\scriptsize 18.6}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 20.8}}$ & \normalsize 97 $\textcolor{red}{\uparrow_{\scriptsize 37.1}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 21.0}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 39.1}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 22.4}}$ & \normalsize 76 $\textcolor{red}{\uparrow_{\scriptsize 17.2}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 16.2}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 36.0}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 21.8}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 29.8}}$ & \normalsize 5 $\textcolor{blue}{\downarrow_{\scriptsize 18.2}}$ & \normalsize 84 $\textcolor{blue}{\downarrow_{\scriptsize 1.9}}$ & \normalsize 72 $\textcolor{red}{\uparrow_{\scriptsize 8.0}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 11.8}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 12.2}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 0.0}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 3.2}}$ \\
% \normalsize Gemini-2.5 Flash & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 41.6}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 20.8}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 40.1}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 21.0}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 39.1}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 22.4}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 41.2}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 16.2}}$ & \normalsize 90 $\textcolor{red}{\uparrow_{\scriptsize 54.0}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 21.8}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 29.8}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 23.2}}$ & \normalsize 98 $\textcolor{red}{\uparrow_{\scriptsize 12.1}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 64.0}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 11.8}}$ & \normalsize 99 $\textcolor{red}{\uparrow_{\scriptsize 11.2}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 0.0}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 3.2}}$ \\
% \rowcolor{gray!10} \normalsize Gemini-2.5 Pro & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 41.6}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 20.8}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 40.1}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 21.0}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 60.9}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 22.4}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 41.2}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 16.2}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 36.0}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 21.8}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 29.8}}$ & \normalsize 8 $\textcolor{blue}{\downarrow_{\scriptsize 15.2}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 14.1}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 36.0}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 11.8}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 12.2}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 0.0}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 3.2}}$ \\
% \normalsize GPT-4o Audio & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 58.4}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 20.8}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 59.9}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 21.0}}$ & \normalsize 30 $\textcolor{blue}{\downarrow_{\scriptsize 30.9}}$ & \normalsize 1 $\textcolor{blue}{\downarrow_{\scriptsize 21.4}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 58.8}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 16.2}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 36.0}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 21.8}}$ & \normalsize 12 $\textcolor{blue}{\downarrow_{\scriptsize 58.2}}$ & \normalsize 1 $\textcolor{blue}{\downarrow_{\scriptsize 22.2}}$ & \normalsize 98 $\textcolor{red}{\uparrow_{\scriptsize 12.1}}$ & \normalsize 78 $\textcolor{red}{\uparrow_{\scriptsize 14.0}}$ & \normalsize 83 $\textcolor{blue}{\downarrow_{\scriptsize 5.2}}$ & \normalsize 69 $\textcolor{blue}{\downarrow_{\scriptsize 18.8}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 0.0}}$ & \normalsize 96 $\textcolor{blue}{\downarrow_{\scriptsize 0.8}}$ \\
% \rowcolor{gray!10} \normalsize GPT-4o Mini Audio & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 58.4}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 20.8}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 59.9}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 21.0}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 60.9}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 22.4}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 58.8}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 16.2}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 36.0}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 21.8}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 70.2}}$ & \normalsize 0 $\textcolor{blue}{\downarrow_{\scriptsize 23.2}}$ & \normalsize 91 $\textcolor{red}{\uparrow_{\scriptsize 5.1}}$ & \normalsize 32 $\textcolor{blue}{\downarrow_{\scriptsize 32.0}}$ & \normalsize 68 $\textcolor{blue}{\downarrow_{\scriptsize 20.2}}$ & \normalsize 52 $\textcolor{blue}{\downarrow_{\scriptsize 35.8}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 0.0}}$ & \normalsize 100 $\textcolor{red}{\uparrow_{\scriptsize 3.2}}$ \\
% \hline
% \normalsize Average & \normalsize 58.4 & \normalsize 20.8 & \normalsize 59.9 & \normalsize 21.0 & \normalsize 60.9 & \normalsize 22.4 & \normalsize 58.8 & \normalsize 16.2 & \normalsize 36.0 & \normalsize 21.8 & \normalsize 70.2 & \normalsize 23.2 & \normalsize 85.9 & \normalsize 64.0 & \normalsize 88.2 & \normalsize 87.8 & \normalsize 100.0 & \normalsize 96.8 \\
% \bottomrule
% \end{tabular}%
% }
% \begin{tablenotes}[flushleft]
% \scriptsize
% \item[] \textbf{Note:} "no aug" indicates the complete disclosure rates before applying a privacy-aware prompt, while "aug" shows rates after applying it. Lower values indicate better performance. Red arrows ($\textcolor{red}{\uparrow}$) indicate worse performance (higher leakage) than average; blue arrows ($\textcolor{blue}{\downarrow}$) indicate better performance (lower leakage) than average. SSN: Social Security Number; Pwd: Phone Password; Setting: Setting of Conversation.
% \end{tablenotes}
% \end{table}



% 0909
% \begin{table}[!htbp]
%     \centering
%     \small
%     \caption{Privacy leakage threat assessment (no-aug only): Inference accuracy when privacy is leaked (\%), with leak rates. Minimum 5 leaked samples required for statistical significance.}
%     \label{tab:leaked_accuracy_threat_no_aug}
%     \renewcommand{\arraystretch}{1.2}
%     \resizebox{\textwidth}{!}{%
%         \begin{tabular}{l|cc|cc|cc|cc|cc|cc|cc|cc|cc}
%             \toprule
%             \multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c|}{\textbf{Bank Account}} & \multicolumn{2}{c|}{\textbf{Driver License}} & \multicolumn{2}{c|}{\textbf{Phone Number}} & \multicolumn{2}{c|}{\textbf{Password}} & \multicolumn{2}{c|}{\textbf{SSN}} & \multicolumn{2}{c|}{\textbf{Address}} & \multicolumn{2}{c|}{\textbf{Age}} & \multicolumn{2}{c|}{\textbf{Ethnicity}} & \multicolumn{2}{c|}{\textbf{Setting} \\
%              & \textbf{\small Acc\%} & \textbf{\small Leak\%} & \textbf{\small Acc\%} & \textbf{\small Leak\%} & \textbf{\small Acc\%} & \textbf{\small Leak\%} & \textbf{\small Acc\%} & \textbf{\small Leak\%} & \textbf{\small Acc\%} & \textbf{\small Leak\%} & \textbf{\small Acc\%} & \textbf{\small Leak\%} & \textbf{\small Acc\%} & \textbf{\small Leak\%} & \textbf{\small Acc\%} & \textbf{\small Leak\%} & \textbf{\small Acc\%} & \textbf{\small Leak\%} \\
%             \midrule
%             \multicolumn{19}{c}{\textbf{Open-source Models}} \\
%             \midrule
%             \rowcolor{gray!10} \normalsize Kimi Audio & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} &  \\
%              \normalsize SALMONN & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} &  \\
%             \rowcolor{gray!10} \normalsize OpenS2S & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} &  \\
%              \normalsize Step Fun & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} &  \\
%             \rowcolor{gray!10} \normalsize Qwen2-Audio & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} &  \\
%              \normalsize Qwen2.5-Omni & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} &  \\
%             \rowcolor{gray!10} \normalsize MiniCPM-o 2.6 & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} &  \\
%              \normalsize Step Audio2 & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} &  \\
%             \rowcolor{gray!10} \normalsize UltraVox & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} &  \\
%             \midrule
%             \multicolumn{19}{c}{\textbf{Closed-source Models}} \\
%             \midrule
%             \rowcolor{gray!10} \normalsize Gemini-1.5 Pro & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} &  \\
%              \normalsize Gemini-2.5 Flash & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} &  \\
%             \rowcolor{gray!10} \normalsize Gemini-2.5 Pro & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} &  \\
%              \normalsize GPT-4o Mini Audio & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} &  \\
%             \rowcolor{gray!10} \normalsize GPT-4o Audio & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} & \normalsize -- & \textcolor{gray}{\normalsize 0.0*} &  \\
%             \midrule
%             \normalsize \textbf{Average} & 0.0 & -- & 0.0 & -- & 0.0 & -- & 0.0 & -- & 0.0 & -- & 0.0 & -- & 0.0 & -- & 0.0 & -- & 0.0 & -- &  \\
%             \bottomrule
%         \end{tabular}%
%     }
%     \vspace{2pt}
%     \footnotesize
%     \begin{tablenotes}[flushleft]
%         \item[] \scriptsize
%         \textbf{Note:} This table shows inference accuracy ONLY for samples where privacy was leaked (leaked\_privacy=true) in no-aug setting. Higher accuracy values indicate greater privacy threat. "Acc\%" = Accuracy when leaked; "Leak\%" = Percentage of samples that leaked privacy. Red arrows ($\textcolor{red}{\uparrow}$) indicate higher threat than average; blue arrows ($\textcolor{blue}{\downarrow}$) indicate lower threat. Gray text with * indicates insufficient leaked samples (<5) for reliable analysis. `--' indicates no data available.
%     \end{tablenotes}
% \end{table}

==> tables/robustness/exp1_robustness.tex <==
\begin{wraptable}{r}{0.54\textwidth}
\small
\centering
\setlength{\tabcolsep}{1.5pt}
\caption{Accuracy of ALLMs under different robustness scenarios averaged over tasks. The highest average accuracy under each scenario is in bold. $\textcolor{red}{\uparrow}$: higher than column average, $\textcolor{blue}{\downarrow}$: lower than column average, subscript is absolute difference. The overall low accuracy highlights the hallucination concerns.}
\rowcolors{2}{gray!10}{white}
\begin{tabular}{l|cccccc}
\toprule
\textbf{Model} & \textbf{AR} & \textbf{AQV} & \textbf{BC} & \textbf{ES} & \textbf{MS} & \textbf{NI} \\
\midrule
\multicolumn{7}{c}{\textbf{Open-source}} \\
\midrule
MiniCPM-o 2.6      & 7.80 $\textcolor{red}{\uparrow_{\scriptsize 1.13}}$ & 7.19 $\textcolor{red}{\uparrow_{\scriptsize 0.25}}$ & 7.92 $\textcolor{red}{\uparrow_{\scriptsize 0.84}}$ & 7.06 $\textcolor{red}{\uparrow_{\scriptsize 0.17}}$ & 6.51 $\textcolor{red}{\uparrow_{\scriptsize 0.24}}$ & 6.18 $\textcolor{blue}{\downarrow_{\scriptsize 0.77}}$ \\
Qwen2.5-Omni       & 8.14 $\textcolor{red}{\uparrow_{\scriptsize 1.47}}$ & 7.10 $\textcolor{red}{\uparrow_{\scriptsize 0.16}}$ & 7.50 $\textcolor{red}{\uparrow_{\scriptsize 0.42}}$ & 7.93 $\textcolor{red}{\uparrow_{\scriptsize 1.04}}$ & 7.12 $\textcolor{red}{\uparrow_{\scriptsize 0.85}}$ & 7.17 $\textcolor{red}{\uparrow_{\scriptsize 0.22}}$ \\
SALMONN            & 2.00 $\textcolor{blue}{\downarrow_{\scriptsize 4.67}}$ & 6.42 $\textcolor{blue}{\downarrow_{\scriptsize 0.52}}$ & 4.57 $\textcolor{blue}{\downarrow_{\scriptsize 2.51}}$ & 2.94 $\textcolor{blue}{\downarrow_{\scriptsize 3.95}}$ & 7.16 $\textcolor{red}{\uparrow_{\scriptsize 0.89}}$ & 6.66 $\textcolor{blue}{\downarrow_{\scriptsize 0.29}}$ \\
Ultravox           & 4.00 $\textcolor{blue}{\downarrow_{\scriptsize 2.67}}$ & 7.53 $\textcolor{red}{\uparrow_{\scriptsize 0.59}}$ & 7.30 $\textcolor{red}{\uparrow_{\scriptsize 0.22}}$ & 6.53 $\textcolor{blue}{\downarrow_{\scriptsize 0.36}}$ & 6.70 $\textcolor{red}{\uparrow_{\scriptsize 0.43}}$ & 7.00 $\textcolor{red}{\uparrow_{\scriptsize 0.05}}$ \\
Step-Fun           & 5.00 $\textcolor{blue}{\downarrow_{\scriptsize 1.67}}$ & 7.48 $\textcolor{red}{\uparrow_{\scriptsize 0.54}}$ & 8.20 $\textcolor{red}{\uparrow_{\scriptsize 1.12}}$ & 7.42 $\textcolor{red}{\uparrow_{\scriptsize 0.53}}$ & 5.89 $\textcolor{blue}{\downarrow_{\scriptsize 0.38}}$ & 7.08 $\textcolor{red}{\uparrow_{\scriptsize 0.13}}$ \\
Kimi Audio         & 5.67 $\textcolor{blue}{\downarrow_{\scriptsize 1.00}}$ & 6.83 $\textcolor{blue}{\downarrow_{\scriptsize 0.11}}$ & 6.00 $\textcolor{blue}{\downarrow_{\scriptsize 1.08}}$ & 6.83 $\textcolor{blue}{\downarrow_{\scriptsize 0.06}}$ & 7.08 $\textcolor{red}{\uparrow_{\scriptsize 0.81}}$ & 6.94 $\textcolor{blue}{\downarrow_{\scriptsize 0.01}}$ \\
Step-Audio2        & 6.18 $\textcolor{blue}{\downarrow_{\scriptsize 0.49}}$ & 6.58 $\textcolor{blue}{\downarrow_{\scriptsize 0.36}}$ & 7.92 $\textcolor{red}{\uparrow_{\scriptsize 0.84}}$ & 6.82 $\textcolor{blue}{\downarrow_{\scriptsize 0.07}}$ & 0.00 $\textcolor{blue}{\downarrow_{\scriptsize 6.27}}$ & 6.78 $\textcolor{blue}{\downarrow_{\scriptsize 0.17}}$ \\
OpenS2S            & 8.25 $\textcolor{red}{\uparrow_{\scriptsize 1.58}}$ & 6.46 $\textcolor{blue}{\downarrow_{\scriptsize 0.48}}$ & 5.17 $\textcolor{blue}{\downarrow_{\scriptsize 1.91}}$ & 6.39 $\textcolor{blue}{\downarrow_{\scriptsize 0.50}}$ & 2.33 $\textcolor{blue}{\downarrow_{\scriptsize 3.94}}$ & 6.25 $\textcolor{blue}{\downarrow_{\scriptsize 0.70}}$ \\
\midrule
\multicolumn{7}{c}{\textbf{Closed-source}} \\
\midrule
Gemini-1.5 Pro     & 8.57 $\textcolor{red}{\uparrow_{\scriptsize 1.90}}$ & 8.21 $\textcolor{red}{\uparrow_{\scriptsize 1.27}}$ & 8.23 $\textcolor{red}{\uparrow_{\scriptsize 1.15}}$ & 8.16 $\textcolor{red}{\uparrow_{\scriptsize 1.27}}$ & 6.09 $\textcolor{blue}{\downarrow_{\scriptsize 0.18}}$ & 7.43 $\textcolor{red}{\uparrow_{\scriptsize 0.48}}$ \\
Gemini-2.5 Flash   & 8.16 $\textcolor{red}{\uparrow_{\scriptsize 1.49}}$ & 8.38 $\textcolor{red}{\uparrow_{\scriptsize 1.44}}$ & 8.28 $\textcolor{red}{\uparrow_{\scriptsize 1.20}}$ & 7.93 $\textcolor{red}{\uparrow_{\scriptsize 1.04}}$ & 6.36 $\textcolor{red}{\uparrow_{\scriptsize 0.09}}$ & 7.76 $\textcolor{red}{\uparrow_{\scriptsize 0.81}}$ \\
Gemini-2.5 Pro     & \textbf{8.88 $\textcolor{red}{\uparrow_{\scriptsize 2.21}}$} & \textbf{8.68 $\textcolor{red}{\uparrow_{\scriptsize 1.74}}$} & \textbf{8.50 $\textcolor{red}{\uparrow_{\scriptsize 1.42}}$} & \textbf{8.18 $\textcolor{red}{\uparrow_{\scriptsize 1.29}}$} & \textbf{7.46 $\textcolor{red}{\uparrow_{\scriptsize 1.19}}$} & 7.71 $\textcolor{red}{\uparrow_{\scriptsize 0.76}}$ \\
GPT-4o Audio       & 5.90 $\textcolor{blue}{\downarrow_{\scriptsize 0.77}}$ & 5.50 $\textcolor{blue}{\downarrow_{\scriptsize 1.44}}$ & 8.33 $\textcolor{red}{\uparrow_{\scriptsize 1.25}}$ & 7.31 $\textcolor{red}{\uparrow_{\scriptsize 0.42}}$ & 7.62 $\textcolor{red}{\uparrow_{\scriptsize 1.35}}$ & 6.27 $\textcolor{blue}{\downarrow_{\scriptsize 0.68}}$ \\
GPT-4o mini Audio  & 8.33 $\textcolor{red}{\uparrow_{\scriptsize 1.66}}$ & 6.90 $\textcolor{blue}{\downarrow_{\scriptsize 0.04}}$ & 7.69 $\textcolor{red}{\uparrow_{\scriptsize 0.61}}$ & 6.00 $\textcolor{blue}{\downarrow_{\scriptsize 0.89}}$ & 5.77 $\textcolor{blue}{\downarrow_{\scriptsize 0.50}}$ & 7.25 $\textcolor{red}{\uparrow_{\scriptsize 0.30}}$ \\
\midrule
\textbf{Average} & 6.67 & 6.94 & 7.08 & 6.89 & 6.27 & 6.95 \\
\bottomrule
\end{tabular}
\begin{tablenotes}[flushleft]
\item[] \hspace{-2pt}\scriptsize 
$\ddagger$: AR: Adversarial Robustness, AQV: Audio Quality Variation, BC: Background Conversation, ES: Environmental Sound, MS: Multiple Speakers, NI: Noise Interference.
\end{tablenotes}
\label{tab:robustness_grouped} 
\end{wraptable}
